Inclusive Deep Inelastic Scattering at High Q2 with Longitudinally Polarised Lepton Beams at HERA

Inclusive e\pmp single and double differential cross sections for neutral and charged current deep inelastic scattering processes are measured with the H1 detector at HERA. The data were taken at a centre-of-mass energy of \surds = 319GeV with a total integrated luminosity of 333.7 pb-1 shared between two lepton beam charges and two longitudinal lepton polarisation modes. The differential cross sections are measured in the range of negative fourmomentum transfer squared, Q2, between 60 and 50 000GeV2, and Bjorken x between 0.0008 and 0.65. The measurements are combined with earlier published unpolarised H1 data to improve statistical precision and used to determine the structure function xF_3^gammaZ. A measurement of the neutral current parity violating structure function F_2^gammaZ is presented for the first time. The polarisation dependence of the charged current total cross section is also measured. The new measurements are well described by a next-to-leading order QCD fit based on all published H1 inclusive cross section data which are used to extract the parton distribution functions of the proton.

==> 515.tex <==
    1 &    60. &    0.800E-03 & 0.750 & 1.474 & 1.655 &  1.02 &  2.09 &  1.66 &  2.86\\
    2 &    90. &    0.118E-02 & 0.750 & 1.477 & 1.658 &  0.83 &  1.98 &  1.61 &  2.68\\
    3 &   100. &    0.131E-02 & 0.750 & 1.365 & 1.533 &  4.00 &  5.50 &  1.76 &  7.03\\
    4 &   100. &    0.200E-02 & 0.494 & 1.278 & 1.331 &  3.42 &  3.30 &  1.82 &  5.09\\
    5 &   120. &    0.158E-02 & 0.750 & 1.428 & 1.603 &  0.95 &  1.91 &  1.56 &  2.65\\
    6 &   120. &    0.200E-02 & 0.593 & 1.352 & 1.442 &  0.70 &  0.96 &  1.68 &  2.06\\
    7 &   120. &    0.320E-02 & 0.371 & 1.214 & 1.239 &  0.96 &  1.12 &  1.54 &  2.13\\
    8 &   150. &    0.197E-02 & 0.750 & 1.348 & 1.513 &  1.06 &  1.97 &  1.54 &  2.71\\
    9 &   150. &    0.320E-02 & 0.463 & 1.225 & 1.268 &  0.60 &  0.89 &  1.57 &  1.90\\
   10 &   150. &    0.500E-02 & 0.296 & 1.106 & 1.120 &  0.72 &  1.16 &  1.55 &  2.06\\
   11 &   150. &    0.800E-02 & 0.185 & 0.949 & 0.953 &  0.98 &  1.74 &  1.63 &  2.58\\
   12 &   150. &    0.130E-01 & 0.114 & 0.811 & 0.813 &  1.38 &  2.99 &  1.86 &  3.79\\
   13 &   200. &    0.263E-02 & 0.750 & 1.273 & 1.429 &  1.32 &  2.04 &  1.53 &  2.88\\
   14 &   200. &    0.320E-02 & 0.618 & 1.244 & 1.336 &  1.08 &  0.88 &  1.58 &  2.11\\
   15 &   200. &    0.500E-02 & 0.395 & 1.104 & 1.131 &  0.77 &  0.95 &  1.54 &  1.96\\
   16 &   200. &    0.800E-02 & 0.247 & 0.954 & 0.962 &  0.80 &  1.28 &  1.55 &  2.16\\
   17 &   200. &    0.130E-01 & 0.152 & 0.797 & 0.800 &  0.90 &  0.86 &  1.51 &  1.96\\
   18 &   200. &    0.200E-01 & 0.099 & 0.697 & 0.698 &  0.98 &  1.06 &  1.52 &  2.10\\
   19 &   200. &    0.320E-01 & 0.062 & 0.580 & 0.581 &  1.11 &  1.40 &  1.56 &  2.37\\
   20 &   200. &    0.500E-01 & 0.040 & 0.526 & 0.526 &  1.31 &  1.71 &  1.70 &  2.75\\
   21 &   200. &    0.800E-01 & 0.025 & 0.438 & 0.439 &  1.38 &  2.14 &  1.83 &  3.14\\
   22 &   200. &    0.130E+00 & 0.015 & 0.362 & 0.362 &  1.68 &  2.32 &  1.78 &  3.38\\
   23 &   200. &    0.180E+00 & 0.011 & 0.308 & 0.308 &  2.27 &  2.97 &  1.89 &  4.18\\
   24 &   250. &    0.328E-02 & 0.750 & 1.261 & 1.415 &  1.51 &  2.04 &  1.53 &  2.96\\
   25 &   250. &    0.500E-02 & 0.494 & 1.122 & 1.169 &  0.90 &  0.88 &  1.53 &  1.98\\
   26 &   250. &    0.800E-02 & 0.309 & 0.968 & 0.981 &  0.87 &  1.01 &  1.55 &  2.04\\
   27 &   250. &    0.130E-01 & 0.190 & 0.818 & 0.821 &  0.96 &  1.21 &  1.60 &  2.22\\
   28 &   250. &    0.200E-01 & 0.124 & 0.691 & 0.692 &  0.98 &  1.21 &  1.56 &  2.21\\
   29 &   250. &    0.320E-01 & 0.077 & 0.586 & 0.587 &  1.04 &  1.31 &  1.58 &  2.30\\
   30 &   250. &    0.500E-01 & 0.049 & 0.497 & 0.497 &  1.19 &  1.28 &  1.59 &  2.36\\
   31 &   250. &    0.800E-01 & 0.031 & 0.427 & 0.427 &  1.22 &  1.11 &  1.75 &  2.40\\
   32 &   250. &    0.130E+00 & 0.019 & 0.362 & 0.362 &  1.26 &  1.85 &  1.62 &  2.76\\
   33 &   250. &    0.180E+00 & 0.014 & 0.309 & 0.309 &  1.77 &  2.92 &  2.14 &  4.03\\
   34 &   250. &    0.250E+00 & 0.010 & 0.228 & 0.228 &  7.45 &  8.60 &  2.04 & 11.56\\
   35 &   250. &    0.400E+00 & 0.006 & 0.139 & 0.139 &  9.27 &  6.80 &  1.68 & 11.62\\
   36 &   300. &    0.394E-02 & 0.750 & 1.207 & 1.355 &  1.73 &  2.02 &  1.52 &  3.06\\
   37 &   300. &    0.500E-02 & 0.593 & 1.152 & 1.228 &  1.50 &  0.93 &  1.54 &  2.34\\
   38 &   300. &    0.800E-02 & 0.371 & 0.989 & 1.009 &  1.01 &  0.88 &  1.52 &  2.03\\
   39 &   300. &    0.130E-01 & 0.228 & 0.827 & 0.832 &  1.02 &  1.09 &  1.56 &  2.16\\
   40 &   300. &    0.200E-01 & 0.148 & 0.706 & 0.708 &  1.13 &  1.05 &  1.57 &  2.20\\
   41 &   300. &    0.320E-01 & 0.093 & 0.593 & 0.593 &  1.19 &  1.15 &  1.57 &  2.28\\
   42 &   300. &    0.500E-01 & 0.059 & 0.502 & 0.503 &  1.29 &  1.39 &  1.63 &  2.50\\
   43 &   300. &    0.800E-01 & 0.037 & 0.423 & 0.423 &  1.38 &  1.38 &  1.75 &  2.62\\
   44 &   300. &    0.130E+00 & 0.023 & 0.358 & 0.358 &  1.38 &  1.97 &  1.62 &  2.90\\
   45 &   300. &    0.180E+00 & 0.016 & 0.298 & 0.298 &  1.90 &  3.26 &  2.35 &  4.44\\
   46 &   300. &    0.250E+00 & 0.012 & 0.282 & 0.282 &  6.84 &  9.40 &  2.38 & 11.86\\
   47 &   300. &    0.400E+00 & 0.007 & 0.148 & 0.148 &  2.26 &  3.54 &  2.93 &  5.12\\
   48 &   400. &    0.525E-02 & 0.750 & 1.149 & 1.290 &  1.87 &  2.03 &  1.51 &  3.15\\
   49 &   400. &    0.800E-02 & 0.494 & 1.042 & 1.086 &  1.24 &  0.93 &  1.53 &  2.18\\
   50 &   400. &    0.130E-01 & 0.304 & 0.859 & 0.870 &  1.20 &  0.95 &  1.53 &  2.16\\
   51 &   400. &    0.200E-01 & 0.198 & 0.716 & 0.720 &  1.24 &  1.22 &  1.58 &  2.35\\
   52 &   400. &    0.320E-01 & 0.124 & 0.604 & 0.605 &  1.31 &  0.97 &  1.55 &  2.25\\
   53 &   400. &    0.500E-01 & 0.079 & 0.499 & 0.499 &  1.45 &  1.07 &  1.54 &  2.37\\
   54 &   400. &    0.800E-01 & 0.049 & 0.422 & 0.422 &  1.55 &  1.03 &  1.66 &  2.50\\
   55 &   400. &    0.130E+00 & 0.030 & 0.367 & 0.367 &  1.55 &  1.56 &  1.60 &  2.71\\
   56 &   400. &    0.180E+00 & 0.022 & 0.308 & 0.308 &  1.98 &  2.69 &  2.24 &  4.02\\
   57 &   400. &    0.250E+00 & 0.016 & 0.241 & 0.241 &  7.58 &  6.70 &  1.86 & 10.28\\
   58 &   400. &    0.400E+00 & 0.010 & 0.148 & 0.148 &  2.60 &  3.30 &  3.16 &  5.26\\
   59 &   500. &    0.656E-02 & 0.750 & 1.054 & 1.184 &  2.06 &  2.00 &  1.51 &  3.24\\
   60 &   500. &    0.800E-02 & 0.618 & 1.003 & 1.077 &  2.06 &  0.97 &  1.52 &  2.74\\
   61 &   500. &    0.130E-01 & 0.380 & 0.895 & 0.914 &  1.47 &  0.93 &  1.52 &  2.31\\
   62 &   500. &    0.200E-01 & 0.247 & 0.732 & 0.738 &  1.46 &  1.12 &  1.56 &  2.41\\
   63 &   500. &    0.320E-01 & 0.154 & 0.622 & 0.624 &  1.50 &  1.04 &  1.56 &  2.40\\
   64 &   500. &    0.500E-01 & 0.099 & 0.542 & 0.542 &  1.59 &  1.10 &  1.57 &  2.49\\
   65 &   500. &    0.800E-01 & 0.062 & 0.428 & 0.428 &  1.79 &  1.12 &  1.64 &  2.67\\
   66 &   500. &    0.130E+00 & 0.038 & 0.372 & 0.373 &  2.07 &  1.48 &  1.63 &  3.02\\
   67 &   500. &    0.180E+00 & 0.027 & 0.328 & 0.328 &  2.25 &  2.01 &  1.71 &  3.46\\
   68 &   500. &    0.250E+00 & 0.020 & 0.255 & 0.255 &  2.67 &  2.63 &  2.40 &  4.45\\
   69 &   500. &    0.400E+00 & 0.012 & 0.139 & 0.139 & 15.38 & 12.00 &  3.68 & 19.85\\
   70 &   500. &    0.650E+00 & 0.008 & 0.027 & 0.027 & 19.28 & 10.50 &  2.05 & 22.05\\
   71 &   650. &    0.853E-02 & 0.750 & 0.991 & 1.113 &  2.34 &  2.03 &  1.50 &  3.44\\
   72 &   650. &    0.130E-01 & 0.494 & 0.904 & 0.942 &  1.66 &  0.98 &  1.51 &  2.44\\
   73 &   650. &    0.200E-01 & 0.321 & 0.766 & 0.777 &  1.72 &  1.03 &  1.53 &  2.52\\
   74 &   650. &    0.320E-01 & 0.201 & 0.650 & 0.654 &  1.76 &  1.31 &  1.59 &  2.71\\
   75 &   650. &    0.500E-01 & 0.128 & 0.541 & 0.542 &  1.86 &  1.11 &  1.59 &  2.69\\
   76 &   650. &    0.800E-01 & 0.080 & 0.432 & 0.433 &  2.11 &  1.12 &  1.59 &  2.87\\
   77 &   650. &    0.130E+00 & 0.049 & 0.356 & 0.356 &  2.44 &  1.58 &  1.63 &  3.33\\
   78 &   650. &    0.180E+00 & 0.036 & 0.326 & 0.326 &  2.52 &  1.87 &  1.62 &  3.53\\
   79 &   650. &    0.250E+00 & 0.026 & 0.252 & 0.253 &  3.20 &  2.62 &  2.25 &  4.71\\
   80 &   650. &    0.400E+00 & 0.016 & 0.119 & 0.119 &  4.91 &  3.66 &  2.73 &  6.71\\
   81 &   800. &    0.105E-01 & 0.750 & 0.960 & 1.077 &  2.71 &  2.07 &  1.50 &  3.73\\
   82 &   800. &    0.130E-01 & 0.608 & 0.894 & 0.957 &  2.78 &  1.08 &  1.51 &  3.34\\
   83 &   800. &    0.200E-01 & 0.395 & 0.737 & 0.754 &  2.00 &  1.05 &  1.50 &  2.71\\
   84 &   800. &    0.320E-01 & 0.247 & 0.635 & 0.640 &  2.10 &  1.30 &  1.54 &  2.91\\
   85 &   800. &    0.500E-01 & 0.158 & 0.554 & 0.556 &  2.16 &  1.03 &  1.52 &  2.84\\
   86 &   800. &    0.800E-01 & 0.099 & 0.431 & 0.432 &  2.44 &  1.15 &  1.58 &  3.12\\
   87 &   800. &    0.130E+00 & 0.061 & 0.355 & 0.356 &  2.94 &  1.55 &  1.61 &  3.69\\
   88 &   800. &    0.180E+00 & 0.044 & 0.318 & 0.318 &  3.11 &  1.93 &  1.63 &  4.01\\
   89 &   800. &    0.250E+00 & 0.032 & 0.239 & 0.239 &  3.67 &  2.29 &  1.85 &  4.70\\
   90 &   800. &    0.400E+00 & 0.020 & 0.131 & 0.131 &  4.90 &  4.15 &  3.27 &  7.20\\
   91 &   800. &    0.650E+00 & 0.012 & 0.015 & 0.015 & 21.79 & 12.50 &  3.33 & 25.34\\
   92 &  1000. &    0.130E-01 & 0.750 & 0.859 & 0.964 &  2.76 &  1.73 &  1.84 &  3.74\\
   93 &  1000. &    0.200E-01 & 0.494 & 0.766 & 0.798 &  2.31 &  1.00 &  1.51 &  2.93\\
   94 &  1000. &    0.320E-01 & 0.309 & 0.655 & 0.664 &  2.33 &  1.09 &  1.51 &  2.98\\
   95 &  1000. &    0.500E-01 & 0.198 & 0.517 & 0.519 &  2.50 &  1.42 &  1.56 &  3.27\\
   96 &  1000. &    0.800E-01 & 0.124 & 0.437 & 0.438 &  2.72 &  1.07 &  1.54 &  3.31\\
   97 &  1000. &    0.130E+00 & 0.076 & 0.365 & 0.365 &  3.22 &  1.51 &  1.59 &  3.90\\
   98 &  1000. &    0.180E+00 & 0.055 & 0.337 & 0.337 &  3.27 &  1.85 &  1.58 &  4.08\\
   99 &  1000. &    0.250E+00 & 0.040 & 0.272 & 0.272 &  3.63 &  2.25 &  1.78 &  4.63\\
  100 &  1000. &    0.400E+00 & 0.025 & 0.128 & 0.128 &  5.31 &  4.30 &  3.15 &  7.53\\
  101 &  1200. &    0.130E-01 & 0.912 & 0.901 & 1.087 &  4.58 &  2.26 &  2.19 &  5.56\\
  102 &  1200. &    0.200E-01 & 0.593 & 0.786 & 0.839 &  2.83 &  1.20 &  1.52 &  3.42\\
  103 &  1200. &    0.320E-01 & 0.371 & 0.680 & 0.694 &  2.62 &  0.96 &  1.51 &  3.17\\
  104 &  1200. &    0.500E-01 & 0.237 & 0.548 & 0.552 &  2.76 &  1.18 &  1.52 &  3.36\\
  105 &  1200. &    0.800E-01 & 0.148 & 0.455 & 0.456 &  2.96 &  1.28 &  1.55 &  3.58\\
  106 &  1200. &    0.130E+00 & 0.091 & 0.356 & 0.357 &  4.06 &  1.56 &  1.54 &  4.62\\
  107 &  1200. &    0.180E+00 & 0.066 & 0.313 & 0.313 &  3.80 &  1.86 &  1.57 &  4.51\\
  108 &  1200. &    0.250E+00 & 0.047 & 0.222 & 0.222 &  4.43 &  2.18 &  1.62 &  5.20\\
  109 &  1200. &    0.400E+00 & 0.030 & 0.127 & 0.127 &  5.64 &  4.32 &  2.91 &  7.67\\
  110 &  1500. &    0.200E-01 & 0.750 & 0.805 & 0.903 &  3.43 &  1.81 &  1.69 &  4.23\\
  111 &  1500. &    0.320E-01 & 0.463 & 0.677 & 0.701 &  3.22 &  1.05 &  1.51 &  3.71\\
  112 &  1500. &    0.500E-01 & 0.296 & 0.553 & 0.560 &  3.20 &  1.18 &  1.51 &  3.73\\
  113 &  1500. &    0.800E-01 & 0.185 & 0.496 & 0.498 &  3.25 &  1.16 &  1.53 &  3.78\\
  114 &  1500. &    0.130E+00 & 0.114 & 0.355 & 0.355 &  4.50 &  1.68 &  1.56 &  5.05\\
  115 &  1500. &    0.180E+00 & 0.082 & 0.297 & 0.297 &  4.47 &  1.94 &  1.57 &  5.12\\
  116 &  1500. &    0.250E+00 & 0.059 & 0.237 & 0.238 &  4.79 &  2.35 &  1.64 &  5.58\\
  117 &  1500. &    0.400E+00 & 0.037 & 0.126 & 0.126 &  7.07 &  3.98 &  2.48 &  8.48\\
  118 &  1500. &    0.650E+00 & 0.023 & 0.015 & 0.015 & 11.78 &  6.39 &  5.38 & 14.44\\
  119 &  2000. &    0.219E-01 & 0.903 & 0.874 & 1.048 &  5.54 &  2.39 &  2.11 &  6.40\\
  120 &  2000. &    0.320E-01 & 0.618 & 0.660 & 0.709 &  3.79 &  1.47 &  1.51 &  4.34\\
  121 &  2000. &    0.500E-01 & 0.395 & 0.550 & 0.563 &  3.90 &  1.10 &  1.51 &  4.32\\
  122 &  2000. &    0.800E-01 & 0.247 & 0.459 & 0.462 &  3.92 &  1.31 &  1.53 &  4.40\\
  123 &  2000. &    0.130E+00 & 0.152 & 0.343 & 0.344 &  4.91 &  1.65 &  1.53 &  5.40\\
  124 &  2000. &    0.180E+00 & 0.110 & 0.295 & 0.295 &  5.26 &  2.17 &  1.60 &  5.92\\
  125 &  2000. &    0.250E+00 & 0.079 & 0.242 & 0.242 &  5.44 &  2.28 &  1.63 &  6.12\\
  126 &  2000. &    0.400E+00 & 0.049 & 0.124 & 0.124 &  6.89 &  3.77 &  2.19 &  8.16\\
  127 &  2000. &    0.650E+00 & 0.030 & 0.011 & 0.011 & 16.87 &  7.88 &  5.62 & 19.45\\
  128 &  3000. &    0.320E-01 & 0.926 & 0.729 & 0.884 &  3.78 &  1.99 &  1.62 &  4.56\\
  129 &  3000. &    0.500E-01 & 0.593 & 0.597 & 0.636 &  3.17 &  1.40 &  1.51 &  3.78\\
  130 &  3000. &    0.800E-01 & 0.371 & 0.500 & 0.510 &  3.45 &  1.26 &  1.50 &  3.97\\
  131 &  3000. &    0.130E+00 & 0.228 & 0.407 & 0.409 &  4.13 &  1.73 &  1.51 &  4.73\\
  132 &  3000. &    0.180E+00 & 0.165 & 0.302 & 0.303 &  4.79 &  1.94 &  1.57 &  5.40\\
  133 &  3000. &    0.250E+00 & 0.119 & 0.240 & 0.240 &  4.98 &  2.25 &  1.63 &  5.70\\
  134 &  3000. &    0.400E+00 & 0.074 & 0.117 & 0.117 &  6.21 &  3.88 &  2.09 &  7.61\\
  135 &  3000. &    0.650E+00 & 0.046 & 0.012 & 0.012 & 13.46 &  7.28 &  4.89 & 16.07\\
  136 &  5000. &    0.547E-01 & 0.903 & 0.638 & 0.765 &  5.03 &  2.13 &  1.60 &  5.69\\
  137 &  5000. &    0.800E-01 & 0.618 & 0.542 & 0.582 &  3.70 &  1.51 &  1.50 &  4.27\\
  138 &  5000. &    0.130E+00 & 0.380 & 0.469 & 0.479 &  4.21 &  1.84 &  1.51 &  4.83\\
  139 &  5000. &    0.180E+00 & 0.274 & 0.381 & 0.385 &  4.81 &  1.89 &  1.49 &  5.38\\
  140 &  5000. &    0.250E+00 & 0.198 & 0.246 & 0.247 &  7.06 &  2.46 &  1.62 &  7.65\\
  141 &  5000. &    0.400E+00 & 0.124 & 0.116 & 0.116 &  7.57 &  3.56 &  1.86 &  8.57\\
  142 &  5000. &    0.650E+00 & 0.076 & 0.015 & 0.015 & 13.11 &  6.48 &  3.37 & 15.00\\
  143 &  8000. &    0.875E-01 & 0.903 & 0.637 & 0.764 &  7.43 &  2.69 &  1.77 &  8.10\\
  144 &  8000. &    0.130E+00 & 0.608 & 0.535 & 0.573 &  5.58 &  2.29 &  1.51 &  6.21\\
  145 &  8000. &    0.180E+00 & 0.439 & 0.382 & 0.394 &  6.27 &  2.20 &  1.50 &  6.81\\
  146 &  8000. &    0.250E+00 & 0.316 & 0.264 & 0.268 &  7.16 &  2.56 &  1.57 &  7.77\\
  147 &  8000. &    0.400E+00 & 0.198 & 0.124 & 0.124 &  9.76 &  4.59 &  2.05 & 10.98\\
  148 &  8000. &    0.650E+00 & 0.122 & 0.013 & 0.013 & 16.85 &  6.70 &  2.81 & 18.35\\
  149 & 12000. &    0.130E+00 & 0.912 & 0.724 & 0.873 & 12.79 &  3.83 &  1.96 & 13.49\\
  150 & 12000. &    0.180E+00 & 0.675 & 0.493 & 0.539 &  7.93 &  2.29 &  1.51 &  8.39\\
  151 & 12000. &    0.250E+00 & 0.474 & 0.309 & 0.321 &  8.79 &  2.58 &  1.53 &  9.29\\
  152 & 12000. &    0.400E+00 & 0.296 & 0.183 & 0.185 & 10.49 &  4.94 &  2.00 & 11.76\\
  153 & 12000. &    0.650E+00 & 0.182 & 0.015 & 0.015 & 23.48 &  6.46 &  2.72 & 24.50\\
  154 & 20000. &    0.250E+00 & 0.800 & 0.466 & 0.534 & 11.99 &  2.91 &  1.68 & 12.45\\
  155 & 20000. &    0.400E+00 & 0.494 & 0.216 & 0.225 & 13.02 &  4.57 &  1.66 & 13.89\\
  156 & 20000. &    0.650E+00 & 0.304 & 0.017 & 0.017 & 31.58 & 14.28 &  3.79 & 34.87\\
  157 & 30000. &    0.400E+00 & 0.750 & 0.205 & 0.230 & 25.51 &  5.61 &  2.22 & 26.22\\
  158 & 30000. &    0.650E+00 & 0.456 & 0.047 & 0.049 & 27.77 &  9.51 &  3.09 & 29.51\\


==> 615.tex <==
    1 &    60. &    0.800E-03 & 0.750 & 1.488 & 1.670 &  0.88 &  2.11 &  1.22 &  2.59\\
    2 &    90. &    0.118E-02 & 0.750 & 1.492 & 1.675 &  0.72 &  1.92 &  1.17 &  2.36\\
    3 &   100. &    0.131E-02 & 0.750 & 1.441 & 1.617 &  1.61 &  3.50 &  1.49 &  4.13\\
    4 &   100. &    0.200E-02 & 0.494 & 1.374 & 1.431 &  1.41 &  2.10 &  1.39 &  2.88\\
    5 &   120. &    0.158E-02 & 0.750 & 1.407 & 1.580 &  0.80 &  1.60 &  1.15 &  2.13\\
    6 &   120. &    0.200E-02 & 0.593 & 1.360 & 1.450 &  0.59 &  0.79 &  1.28 &  1.61\\
    7 &   120. &    0.320E-02 & 0.371 & 1.220 & 1.245 &  0.76 &  0.92 &  1.12 &  1.64\\
    8 &   150. &    0.197E-02 & 0.750 & 1.381 & 1.551 &  0.91 &  1.65 &  1.13 &  2.20\\
    9 &   150. &    0.320E-02 & 0.520 & 1.231 & 1.290 &  1.81 &  4.90 &  1.30 &  5.38\\
   10 &   150. &    0.320E-02 & 0.463 & 1.236 & 1.280 &  0.50 &  0.79 &  1.15 &  1.48\\
   11 &   150. &    0.500E-02 & 0.296 & 1.089 & 1.102 &  0.55 &  0.95 &  1.09 &  1.54\\
   12 &   150. &    0.800E-02 & 0.185 & 0.954 & 0.958 &  0.78 &  1.51 &  1.16 &  2.06\\
   13 &   150. &    0.130E-01 & 0.114 & 0.798 & 0.799 &  1.28 &  2.74 &  1.68 &  3.46\\
   14 &   200. &    0.263E-02 & 0.750 & 1.304 & 1.464 &  1.11 &  1.68 &  1.12 &  2.31\\
   15 &   200. &    0.320E-02 & 0.618 & 1.244 & 1.336 &  0.92 &  0.76 &  1.19 &  1.69\\
   16 &   200. &    0.500E-02 & 0.443 & 1.086 & 1.121 &  1.81 &  4.70 &  1.26 &  5.19\\
   17 &   200. &    0.500E-02 & 0.395 & 1.103 & 1.130 &  0.63 &  0.83 &  1.11 &  1.52\\
   18 &   200. &    0.800E-02 & 0.247 & 0.950 & 0.958 &  0.60 &  1.06 &  1.11 &  1.65\\
   19 &   200. &    0.130E-01 & 0.152 & 0.802 & 0.804 &  0.70 &  0.70 &  1.08 &  1.46\\
   20 &   200. &    0.200E-01 & 0.099 & 0.701 & 0.702 &  0.76 &  0.92 &  1.08 &  1.61\\
   21 &   200. &    0.320E-01 & 0.062 & 0.591 & 0.591 &  0.88 &  1.19 &  1.10 &  1.84\\
   22 &   200. &    0.500E-01 & 0.040 & 0.518 & 0.518 &  0.99 &  1.60 &  1.36 &  2.32\\
   23 &   200. &    0.800E-01 & 0.025 & 0.432 & 0.432 &  1.10 &  1.72 &  1.40 &  2.48\\
   24 &   200. &    0.130E+00 & 0.015 & 0.360 & 0.360 &  1.30 &  1.94 &  1.35 &  2.69\\
   25 &   200. &    0.180E+00 & 0.011 & 0.314 & 0.314 &  1.99 &  3.10 &  1.49 &  3.97\\
   26 &   200. &    0.250E+00 & 0.008 & 0.269 & 0.269 &  3.63 &  4.20 &  2.63 &  6.14\\
   27 &   200. &    0.400E+00 & 0.005 & 0.135 & 0.135 &  4.67 &  4.29 &  4.86 &  8.00\\
   28 &   250. &    0.328E-02 & 0.750 & 1.277 & 1.434 &  1.26 &  1.68 &  1.12 &  2.38\\
   29 &   250. &    0.500E-02 & 0.554 & 1.103 & 1.165 &  2.31 &  4.90 &  1.29 &  5.57\\
   30 &   250. &    0.500E-02 & 0.494 & 1.127 & 1.174 &  0.75 &  0.74 &  1.11 &  1.53\\
   31 &   250. &    0.800E-02 & 0.309 & 0.963 & 0.976 &  0.68 &  0.85 &  1.10 &  1.55\\
   32 &   250. &    0.130E-01 & 0.190 & 0.815 & 0.819 &  0.74 &  1.01 &  1.13 &  1.69\\
   33 &   250. &    0.200E-01 & 0.124 & 0.700 & 0.702 &  0.74 &  1.10 &  1.12 &  1.74\\
   34 &   250. &    0.320E-01 & 0.077 & 0.583 & 0.584 &  0.80 &  1.04 &  1.12 &  1.73\\
   35 &   250. &    0.500E-01 & 0.049 & 0.508 & 0.508 &  0.87 &  1.04 &  1.20 &  1.81\\
   36 &   250. &    0.800E-01 & 0.031 & 0.434 & 0.434 &  0.91 &  0.96 &  1.35 &  1.89\\
   37 &   250. &    0.130E+00 & 0.019 & 0.360 & 0.360 &  0.99 &  1.57 &  1.19 &  2.21\\
   38 &   250. &    0.180E+00 & 0.014 & 0.299 & 0.299 &  1.62 &  2.94 &  1.80 &  3.81\\
   39 &   250. &    0.250E+00 & 0.010 & 0.260 & 0.260 &  2.14 &  3.68 &  2.33 &  4.86\\
   40 &   250. &    0.400E+00 & 0.006 & 0.135 & 0.135 &  3.18 &  3.97 &  4.38 &  6.71\\
   41 &   300. &    0.394E-02 & 0.750 & 1.214 & 1.363 &  1.40 &  1.68 &  1.10 &  2.45\\
   42 &   300. &    0.500E-02 & 0.675 & 1.147 & 1.253 &  3.39 &  5.20 &  1.46 &  6.38\\
   43 &   300. &    0.500E-02 & 0.593 & 1.143 & 1.218 &  1.25 &  0.86 &  1.14 &  1.90\\
   44 &   300. &    0.800E-02 & 0.416 & 0.974 & 1.001 &  2.42 &  4.90 &  1.24 &  5.60\\
   45 &   300. &    0.800E-02 & 0.371 & 0.979 & 0.999 &  0.85 &  0.76 &  1.09 &  1.58\\
   46 &   300. &    0.130E-01 & 0.228 & 0.817 & 0.822 &  0.80 &  0.87 &  1.11 &  1.62\\
   47 &   300. &    0.200E-01 & 0.148 & 0.714 & 0.716 &  0.88 &  0.85 &  1.10 &  1.65\\
   48 &   300. &    0.320E-01 & 0.093 & 0.593 & 0.593 &  0.91 &  1.00 &  1.12 &  1.76\\
   49 &   300. &    0.500E-01 & 0.059 & 0.496 & 0.496 &  0.98 &  1.11 &  1.15 &  1.88\\
   50 &   300. &    0.800E-01 & 0.037 & 0.442 & 0.442 &  1.01 &  1.23 &  1.35 &  2.09\\
   51 &   300. &    0.130E+00 & 0.023 & 0.365 & 0.365 &  1.06 &  1.71 &  1.21 &  2.35\\
   52 &   300. &    0.180E+00 & 0.016 & 0.308 & 0.308 &  1.67 &  3.11 &  2.03 &  4.07\\
   53 &   300. &    0.250E+00 & 0.012 & 0.258 & 0.258 &  2.14 &  4.45 &  2.56 &  5.57\\
   54 &   300. &    0.400E+00 & 0.007 & 0.150 & 0.150 &  1.79 &  3.18 &  3.01 &  4.74\\
   55 &   400. &    0.525E-02 & 0.750 & 1.179 & 1.323 &  1.49 &  1.73 &  1.08 &  2.53\\
   56 &   400. &    0.800E-02 & 0.554 & 0.963 & 1.017 &  3.12 &  4.90 &  1.26 &  5.94\\
   57 &   400. &    0.800E-02 & 0.494 & 1.008 & 1.050 &  1.05 &  0.78 &  1.10 &  1.71\\
   58 &   400. &    0.130E-01 & 0.304 & 0.857 & 0.869 &  0.93 &  0.81 &  1.09 &  1.65\\
   59 &   400. &    0.200E-01 & 0.198 & 0.717 & 0.720 &  0.95 &  1.01 &  1.13 &  1.79\\
   60 &   400. &    0.320E-01 & 0.124 & 0.601 & 0.602 &  1.02 &  0.85 &  1.11 &  1.73\\
   61 &   400. &    0.500E-01 & 0.079 & 0.503 & 0.503 &  1.10 &  0.98 &  1.16 &  1.87\\
   62 &   400. &    0.800E-01 & 0.049 & 0.435 & 0.436 &  1.17 &  0.90 &  1.32 &  1.98\\
   63 &   400. &    0.130E+00 & 0.030 & 0.360 & 0.360 &  1.17 &  1.33 &  1.16 &  2.12\\
   64 &   400. &    0.180E+00 & 0.022 & 0.308 & 0.308 &  1.85 &  2.65 &  2.07 &  3.84\\
   65 &   400. &    0.250E+00 & 0.016 & 0.245 & 0.245 &  2.39 &  3.23 &  2.20 &  4.58\\
   66 &   400. &    0.400E+00 & 0.010 & 0.152 & 0.152 &  2.04 &  2.61 &  3.13 &  4.56\\
   67 &   500. &    0.656E-02 & 0.750 & 1.049 & 1.177 &  1.67 &  1.70 &  1.08 &  2.62\\
   68 &   500. &    0.800E-02 & 0.675 & 1.023 & 1.118 &  4.21 &  5.00 &  1.27 &  6.66\\
   69 &   500. &    0.800E-02 & 0.618 & 0.999 & 1.072 &  1.73 &  0.93 &  1.10 &  2.25\\
   70 &   500. &    0.130E-01 & 0.426 & 0.889 & 0.915 &  3.33 &  5.00 &  1.25 &  6.14\\
   71 &   500. &    0.130E-01 & 0.380 & 0.875 & 0.895 &  1.22 &  0.83 &  1.09 &  1.83\\
   72 &   500. &    0.200E-01 & 0.247 & 0.744 & 0.750 &  1.15 &  0.93 &  1.11 &  1.85\\
   73 &   500. &    0.320E-01 & 0.154 & 0.616 & 0.618 &  1.20 &  0.90 &  1.11 &  1.86\\
   74 &   500. &    0.500E-01 & 0.099 & 0.526 & 0.527 &  1.25 &  1.01 &  1.17 &  1.99\\
   75 &   500. &    0.800E-01 & 0.062 & 0.442 & 0.442 &  1.34 &  0.93 &  1.19 &  2.02\\
   76 &   500. &    0.130E+00 & 0.038 & 0.373 & 0.373 &  1.54 &  1.28 &  1.25 &  2.36\\
   77 &   500. &    0.180E+00 & 0.027 & 0.306 & 0.306 &  1.72 &  1.67 &  1.25 &  2.71\\
   78 &   500. &    0.250E+00 & 0.020 & 0.250 & 0.250 &  2.12 &  2.27 &  2.42 &  3.94\\
   79 &   500. &    0.400E+00 & 0.012 & 0.159 & 0.159 &  5.20 &  5.86 &  4.81 &  9.19\\
   80 &   650. &    0.853E-02 & 0.750 & 0.997 & 1.119 &  1.90 &  1.83 &  1.07 &  2.85\\
   81 &   650. &    0.130E-01 & 0.554 & 0.891 & 0.941 &  4.03 &  3.80 &  1.37 &  5.70\\
   82 &   650. &    0.130E-01 & 0.494 & 0.860 & 0.896 &  1.40 &  0.81 &  1.08 &  1.94\\
   83 &   650. &    0.200E-01 & 0.360 & 0.706 & 0.719 &  4.14 &  3.70 &  1.23 &  5.68\\
   84 &   650. &    0.200E-01 & 0.321 & 0.737 & 0.748 &  1.45 &  0.97 &  1.10 &  2.06\\
   85 &   650. &    0.320E-01 & 0.201 & 0.637 & 0.640 &  1.38 &  1.09 &  1.13 &  2.09\\
   86 &   650. &    0.500E-01 & 0.128 & 0.521 & 0.522 &  1.46 &  0.99 &  1.14 &  2.10\\
   87 &   650. &    0.800E-01 & 0.080 & 0.426 & 0.427 &  1.59 &  1.00 &  1.19 &  2.22\\
   88 &   650. &    0.130E+00 & 0.049 & 0.381 & 0.381 &  1.80 &  1.33 &  1.24 &  2.56\\
   89 &   650. &    0.180E+00 & 0.036 & 0.327 & 0.327 &  1.92 &  1.67 &  1.27 &  2.84\\
   90 &   650. &    0.250E+00 & 0.026 & 0.245 & 0.245 &  2.37 &  2.30 &  2.13 &  3.93\\
   91 &   650. &    0.400E+00 & 0.016 & 0.137 & 0.137 &  3.48 &  3.22 &  3.06 &  5.65\\
   92 &   650. &    0.650E+00 & 0.010 & 0.022 & 0.022 & 14.12 &  7.79 &  5.67 & 17.10\\
   93 &   800. &    0.105E-01 & 0.750 & 0.928 & 1.042 &  2.28 &  1.93 &  1.09 &  3.18\\
   94 &   800. &    0.130E-01 & 0.675 & 0.987 & 1.079 &  5.03 &  4.40 &  1.44 &  6.84\\
   95 &   800. &    0.130E-01 & 0.608 & 0.833 & 0.892 &  2.27 &  1.04 &  1.10 &  2.73\\
   96 &   800. &    0.200E-01 & 0.443 & 0.778 & 0.803 &  4.65 &  4.00 &  1.37 &  6.29\\
   97 &   800. &    0.200E-01 & 0.395 & 0.715 & 0.732 &  1.66 &  0.95 &  1.08 &  2.20\\
   98 &   800. &    0.320E-01 & 0.247 & 0.621 & 0.626 &  1.63 &  1.06 &  1.08 &  2.22\\
   99 &   800. &    0.500E-01 & 0.158 & 0.534 & 0.536 &  1.71 &  0.96 &  1.09 &  2.24\\
  100 &   800. &    0.800E-01 & 0.099 & 0.458 & 0.458 &  1.80 &  1.07 &  1.16 &  2.39\\
  101 &   800. &    0.130E+00 & 0.061 & 0.360 & 0.360 &  2.11 &  1.39 &  1.23 &  2.81\\
  102 &   800. &    0.180E+00 & 0.044 & 0.327 & 0.327 &  2.22 &  1.63 &  1.18 &  2.99\\
  103 &   800. &    0.250E+00 & 0.032 & 0.239 & 0.239 &  2.67 &  2.13 &  1.70 &  3.81\\
  104 &   800. &    0.400E+00 & 0.020 & 0.129 & 0.129 &  3.89 &  3.44 &  3.14 &  6.07\\
  105 &   800. &    0.650E+00 & 0.012 & 0.019 & 0.019 & 12.37 &  7.21 &  5.52 & 15.35\\
  106 &  1000. &    0.130E-01 & 0.750 & 0.824 & 0.925 &  2.34 &  1.56 &  1.41 &  3.14\\
  107 &  1000. &    0.200E-01 & 0.554 & 0.744 & 0.785 &  5.44 &  3.70 &  1.26 &  6.70\\
  108 &  1000. &    0.200E-01 & 0.494 & 0.737 & 0.768 &  1.92 &  0.93 &  1.09 &  2.40\\
  109 &  1000. &    0.320E-01 & 0.309 & 0.625 & 0.634 &  1.82 &  1.02 &  1.09 &  2.35\\
  110 &  1000. &    0.500E-01 & 0.198 & 0.534 & 0.537 &  1.88 &  1.28 &  1.09 &  2.53\\
  111 &  1000. &    0.800E-01 & 0.124 & 0.444 & 0.445 &  2.04 &  1.05 &  1.09 &  2.54\\
  112 &  1000. &    0.130E+00 & 0.076 & 0.362 & 0.363 &  2.53 &  1.34 &  1.19 &  3.10\\
  113 &  1000. &    0.180E+00 & 0.055 & 0.310 & 0.310 &  2.60 &  1.48 &  1.11 &  3.19\\
  114 &  1000. &    0.250E+00 & 0.040 & 0.249 & 0.249 &  2.90 &  1.91 &  1.41 &  3.75\\
  115 &  1000. &    0.400E+00 & 0.025 & 0.128 & 0.128 &  4.70 &  3.30 &  2.73 &  6.36\\
  116 &  1000. &    0.650E+00 & 0.015 & 0.018 & 0.018 & 14.30 &  7.76 &  5.63 & 17.22\\
  117 &  1200. &    0.130E-01 & 0.912 & 0.850 & 1.025 &  4.33 &  2.32 &  2.16 &  5.37\\
  118 &  1200. &    0.200E-01 & 0.675 & 0.729 & 0.797 &  7.24 &  3.50 &  1.24 &  8.13\\
  119 &  1200. &    0.200E-01 & 0.593 & 0.728 & 0.776 &  2.41 &  1.11 &  1.09 &  2.87\\
  120 &  1200. &    0.320E-01 & 0.416 & 0.635 & 0.653 &  6.45 &  3.50 &  1.23 &  7.44\\
  121 &  1200. &    0.320E-01 & 0.371 & 0.618 & 0.631 &  2.23 &  0.92 &  1.08 &  2.64\\
  122 &  1200. &    0.500E-01 & 0.237 & 0.512 & 0.516 &  2.15 &  1.10 &  1.08 &  2.65\\
  123 &  1200. &    0.800E-01 & 0.148 & 0.442 & 0.443 &  2.26 &  1.06 &  1.11 &  2.73\\
  124 &  1200. &    0.130E+00 & 0.091 & 0.367 & 0.368 &  2.71 &  1.41 &  1.13 &  3.26\\
  125 &  1200. &    0.180E+00 & 0.066 & 0.325 & 0.325 &  3.01 &  1.46 &  1.16 &  3.55\\
  126 &  1200. &    0.250E+00 & 0.047 & 0.255 & 0.255 &  3.28 &  1.93 &  1.30 &  4.02\\
  127 &  1200. &    0.400E+00 & 0.030 & 0.115 & 0.115 &  4.69 &  3.45 &  2.87 &  6.49\\
  128 &  1200. &    0.650E+00 & 0.018 & 0.021 & 0.021 & 15.10 &  8.73 &  5.31 & 18.23\\
  129 &  1500. &    0.200E-01 & 0.850 & 0.797 & 0.933 &  9.16 &  4.80 &  1.49 & 10.45\\
  130 &  1500. &    0.200E-01 & 0.750 & 0.700 & 0.785 &  3.03 &  1.70 &  1.22 &  3.68\\
  131 &  1500. &    0.320E-01 & 0.520 & 0.570 & 0.597 &  8.18 &  4.00 &  1.30 &  9.19\\
  132 &  1500. &    0.320E-01 & 0.463 & 0.599 & 0.621 &  2.89 &  1.01 &  1.08 &  3.24\\
  133 &  1500. &    0.500E-01 & 0.296 & 0.536 & 0.543 &  2.44 &  0.99 &  1.06 &  2.84\\
  134 &  1500. &    0.800E-01 & 0.185 & 0.447 & 0.449 &  2.61 &  1.13 &  1.10 &  3.05\\
  135 &  1500. &    0.130E+00 & 0.114 & 0.343 & 0.343 &  3.15 &  1.40 &  1.11 &  3.62\\
  136 &  1500. &    0.180E+00 & 0.082 & 0.314 & 0.315 &  3.27 &  1.52 &  1.16 &  3.79\\
  137 &  1500. &    0.250E+00 & 0.059 & 0.235 & 0.235 &  3.59 &  2.06 &  1.32 &  4.34\\
  138 &  1500. &    0.400E+00 & 0.037 & 0.119 & 0.119 &  4.88 &  3.08 &  2.23 &  6.19\\
  139 &  1500. &    0.650E+00 & 0.023 & 0.016 & 0.016 &  9.84 &  5.94 &  5.25 & 12.64\\
  140 &  2000. &    0.219E-01 & 0.903 & 0.709 & 0.851 &  5.57 &  2.60 &  1.80 &  6.40\\
  141 &  2000. &    0.320E-01 & 0.675 & 0.608 & 0.665 &  9.04 &  4.00 &  1.26 &  9.97\\
  142 &  2000. &    0.320E-01 & 0.618 & 0.571 & 0.613 &  3.36 &  1.45 &  1.09 &  3.82\\
  143 &  2000. &    0.500E-01 & 0.443 & 0.530 & 0.547 &  8.79 &  4.00 &  1.25 &  9.74\\
  144 &  2000. &    0.500E-01 & 0.395 & 0.523 & 0.536 &  3.28 &  1.12 &  1.09 &  3.63\\
  145 &  2000. &    0.800E-01 & 0.247 & 0.425 & 0.428 &  3.02 &  1.21 &  1.08 &  3.43\\
  146 &  2000. &    0.130E+00 & 0.152 & 0.351 & 0.352 &  3.77 &  1.55 &  1.12 &  4.23\\
  147 &  2000. &    0.180E+00 & 0.110 & 0.315 & 0.315 &  3.84 &  1.54 &  1.16 &  4.29\\
  148 &  2000. &    0.250E+00 & 0.079 & 0.239 & 0.239 &  4.03 &  2.09 &  1.32 &  4.72\\
  149 &  2000. &    0.400E+00 & 0.049 & 0.122 & 0.122 &  5.27 &  3.31 &  2.16 &  6.58\\
  150 &  2000. &    0.650E+00 & 0.030 & 0.016 & 0.016 & 10.68 &  6.13 &  5.30 & 13.41\\
  151 &  3000. &    0.320E-01 & 0.926 & 0.601 & 0.730 &  3.71 &  1.97 &  1.33 &  4.41\\
  152 &  3000. &    0.500E-01 & 0.675 & 0.503 & 0.549 &  7.38 &  3.80 &  1.30 &  8.40\\
  153 &  3000. &    0.500E-01 & 0.593 & 0.519 & 0.554 &  2.79 &  1.32 &  1.08 &  3.27\\
  154 &  3000. &    0.800E-01 & 0.416 & 0.452 & 0.464 &  7.75 &  4.00 &  1.20 &  8.81\\
  155 &  3000. &    0.800E-01 & 0.371 & 0.440 & 0.449 &  2.99 &  1.23 &  1.09 &  3.42\\
  156 &  3000. &    0.130E+00 & 0.228 & 0.342 & 0.345 &  3.35 &  1.51 &  1.07 &  3.83\\
  157 &  3000. &    0.180E+00 & 0.165 & 0.309 & 0.310 &  3.91 &  1.87 &  1.20 &  4.50\\
  158 &  3000. &    0.250E+00 & 0.119 & 0.223 & 0.223 &  3.86 &  1.80 &  1.21 &  4.43\\
  159 &  3000. &    0.400E+00 & 0.074 & 0.120 & 0.120 &  4.70 &  3.12 &  1.81 &  5.92\\
  160 &  3000. &    0.650E+00 & 0.046 & 0.013 & 0.013 & 10.10 &  6.09 &  4.54 & 12.64\\
  161 &  5000. &    0.547E-01 & 0.903 & 0.479 & 0.575 &  5.03 &  2.23 &  1.47 &  5.69\\
  162 &  5000. &    0.800E-01 & 0.675 & 0.345 & 0.377 & 10.52 &  4.40 &  1.35 & 11.48\\
  163 &  5000. &    0.800E-01 & 0.618 & 0.415 & 0.446 &  3.42 &  1.50 &  1.09 &  3.89\\
  164 &  5000. &    0.130E+00 & 0.426 & 0.384 & 0.395 & 10.51 &  4.80 &  1.29 & 11.62\\
  165 &  5000. &    0.130E+00 & 0.380 & 0.341 & 0.349 &  4.04 &  1.79 &  1.09 &  4.55\\
  166 &  5000. &    0.180E+00 & 0.274 & 0.281 & 0.284 &  4.25 &  1.75 &  1.04 &  4.71\\
  167 &  5000. &    0.250E+00 & 0.198 & 0.230 & 0.231 &  4.91 &  2.29 &  1.18 &  5.54\\
  168 &  5000. &    0.400E+00 & 0.124 & 0.114 & 0.114 &  5.96 &  2.95 &  1.37 &  6.79\\
  169 &  5000. &    0.650E+00 & 0.076 & 0.011 & 0.011 & 13.41 &  5.89 &  3.34 & 15.03\\
  170 &  8000. &    0.875E-01 & 0.903 & 0.360 & 0.432 &  8.63 &  2.86 &  2.07 &  9.33\\
  171 &  8000. &    0.130E+00 & 0.675 & 0.278 & 0.304 & 16.65 &  4.70 &  1.27 & 17.35\\
  172 &  8000. &    0.130E+00 & 0.608 & 0.306 & 0.328 &  5.89 &  2.30 &  1.09 &  6.42\\
  173 &  8000. &    0.180E+00 & 0.493 & 0.276 & 0.288 & 15.71 &  6.10 &  1.43 & 16.92\\
  174 &  8000. &    0.180E+00 & 0.439 & 0.288 & 0.297 &  5.88 &  2.32 &  1.09 &  6.41\\
  175 &  8000. &    0.250E+00 & 0.355 & 0.269 & 0.274 & 15.20 &  6.60 &  1.55 & 16.65\\
  176 &  8000. &    0.250E+00 & 0.316 & 0.220 & 0.223 &  7.36 &  2.65 &  1.19 &  7.91\\
  177 &  8000. &    0.400E+00 & 0.198 & 0.099 & 0.100 &  8.25 &  3.86 &  1.52 &  9.23\\
  178 &  8000. &    0.650E+00 & 0.122 & 0.016 & 0.016 & 13.01 &  6.71 &  2.92 & 14.93\\
  179 & 12000. &    0.130E+00 & 0.912 & 0.218 & 0.263 & 19.69 &  5.08 &  1.67 & 20.41\\
  180 & 12000. &    0.180E+00 & 0.750 & 0.151 & 0.170 & 34.60 &  3.80 &  1.49 & 34.84\\
  181 & 12000. &    0.180E+00 & 0.675 & 0.222 & 0.243 &  9.79 &  2.29 &  1.20 & 10.13\\
  182 & 12000. &    0.250E+00 & 0.532 & 0.124 & 0.130 & 32.46 &  6.10 &  1.31 & 33.06\\
  183 & 12000. &    0.250E+00 & 0.474 & 0.146 & 0.152 & 10.57 &  2.65 &  1.12 & 10.95\\
  184 & 12000. &    0.400E+00 & 0.296 & 0.086 & 0.087 & 11.90 &  4.23 &  1.40 & 12.71\\
  185 & 12000. &    0.650E+00 & 0.182 & 0.017 & 0.017 & 18.03 &  6.93 &  2.45 & 19.47\\
  186 & 20000. &    0.250E+00 & 0.887 & 0.091 & 0.109 & 61.47 &  5.10 &  1.74 & 61.70\\
  187 & 20000. &    0.250E+00 & 0.800 & 0.122 & 0.140 & 17.86 &  2.84 &  1.24 & 18.12\\
  188 & 20000. &    0.400E+00 & 0.554 & 0.137 & 0.145 & 36.30 &  9.60 &  1.54 & 37.58\\
  189 & 20000. &    0.400E+00 & 0.494 & 0.080 & 0.084 & 17.65 &  4.50 &  1.26 & 18.26\\
  190 & 20000. &    0.650E+00 & 0.304 & 0.012 & 0.012 & 33.26 & 13.49 &  3.18 & 36.03\\
  191 & 30000. &    0.400E+00 & 0.850 & 0.182 & 0.213 & 71.99 &  9.40 &  1.56 & 72.62\\
  192 & 30000. &    0.400E+00 & 0.750 & 0.081 & 0.091 & 32.53 &  5.10 &  1.20 & 32.95\\
  193 & 30000. &    0.650E+00 & 0.456 & 0.008 & 0.009 & 70.24 &  9.57 &  2.44 & 70.93\\


==> KncDq2.tex <==
\begin{table}[htb] 
\begin{center} 
\footnotesize 
\begin{tabular}{|r|l|l||r|r|r|r|r|r|r|r|r|} 
\hline 
$Q^2$                & ${\rm d}\sigma_{NC}/{\rm d}Q^2$      &   $k_{\rm cor}$           & 
$\delta_{stat}$      & $\delta_{unc}$         &   $\delta_{cor}$          & 
$\delta_{tot}$       & $\delta_{cor}^{E^+}$   & $\delta_{cor}^{	heta^+}$ & $\delta_{cor}^{h^+}$& 
$\delta_{cor}^{N^+}$ & $\delta_{cor}^{B^+}$ \\ 
$(\rm GeV^2)$ &$(\rm pb / \rm GeV^2)$ &   & 
$(%)$ &$(%)$ &$(%)$ &$(%)$ &$(%)$ & 
$(%)$ &$(%)$ &$(%)$ &$(%)$ \\ 
&$y<0.9$&&&&&&&&&&\\ 
\hline 
     200 & 1.824 \cdot 10^{ 1} &    0.000 &     0.40 &    0.80  &    0.70 &    1.20 &   -0.40 &   -0.60 &    0.00 &    0.10 &  -0.100    -0.1 \\ 
     250 & 1.079 \cdot 10^{ 1} &    0.000 &     0.40 &    1.10  &    0.80 &    1.50 &    0.60 &   -0.50 &    0.00 &    0.10 &  -0.000    -0.0 \\ 
     300 & 6.919 \cdot 10^{ 0} &    0.000 &     0.50 &    1.10  &    1.00 &    1.60 &    0.80 &   -0.60 &    0.00 &    0.00 &  -0.000    -0.0 \\ 
     400 & 3.496 \cdot 10^{ 0} &    0.000 &     0.60 &    0.90  &    0.90 &    1.40 &    0.80 &   -0.40 &    0.00 &    0.00 &  -0.000    -0.0 \\ 
     500 & 2.074 \cdot 10^{ 0} &    0.000 &     0.70 &    0.90  &    0.90 &    1.50 &    0.80 &   -0.40 &    0.00 &    0.00 &  -0.000    -0.0 \\ 
     650 & 1.082 \cdot 10^{ 0} &    0.000 &     0.90 &    0.90  &    1.00 &    1.60 &    0.90 &   -0.40 &    0.00 &    0.10 &  -0.000    -0.0 \\ 
     800 & 0.642 \cdot 10^{ 0} &    0.000 &     1.00 &    0.90  &    0.90 &    1.60 &    0.80 &   -0.30 &    0.00 &    0.10 &  -0.000    -0.0 \\ 
    1000 & 0.371 \cdot 10^{ 0} &    0.000 &     1.20 &    0.90  &    0.80 &    1.70 &    0.80 &   -0.30 &    0.00 &    0.10 &  -0.200    -0.2 \\ 
    1200 & 0.233 \cdot 10^{ 0} &    0.000 &     1.40 &    1.10  &    0.90 &    2.00 &    0.80 &   -0.20 &    0.00 &    0.10 &  -0.100    -0.1 \\ 
    1500 & 0.135 \cdot 10^{ 0} &    0.000 &     1.70 &    1.10  &    0.90 &    2.20 &    0.80 &   -0.20 &    0.00 &    0.10 &  -0.200    -0.2 \\ 
    2000 & 0.621 \cdot 10^{-1} &    0.000 &     2.10 &    1.50  &    1.00 &    2.80 &    0.90 &   -0.20 &    0.00 &    0.10 &  -0.200    -0.2 \\ 
    3000 & 0.224 \cdot 10^{-1} &    0.000 &     1.90 &    1.50  &    0.80 &    2.60 &    0.80 &   -0.20 &    0.00 &    0.00 &  -0.100    -0.1 \\ 
    5000 & 0.599 \cdot 10^{-2} &    0.000 &     2.50 &    1.50  &    0.70 &    3.00 &    0.70 &   -0.20 &    0.00 &    0.00 &  -0.200    -0.2 \\ 
    8000 & 0.160 \cdot 10^{-2} &    0.000 &     3.80 &    2.00  &    1.00 &    4.40 &    0.90 &   -0.10 &    0.00 &    0.00 &  -0.200    -0.2 \\ 
   12000 & 0.567 \cdot 10^{-3} &    0.000 &     5.80 &    2.40  &    1.10 &    6.30 &    1.10 &    0.00 &    0.00 &    0.10 &  -0.300    -0.3 \\ 
   20000 & 0.121 \cdot 10^{-3} &    0.000 &     9.80 &    3.50  &    1.70 &   10.60 &    1.50 &    0.10 &    0.00 &    0.00 &  -0.700    -0.7 \\ 
   30000 & 0.188 \cdot 10^{-4} &    0.000 &    25.70 &    5.60  &    3.00 &   26.50 &    2.70 &    0.30 &    0.00 &    0.10 &  -1.300    -1.3 \\ 
   50000 & 0.269 \cdot 10^{-5} &    0.000 &    57.80 &    6.40  &    3.00 &   58.20 &    3.00 &    0.50 &   -0.00 &   -0.00 &  -0.000    -0.0 \\ 
\hline 
\end{tabular} 
\end{center} 
\caption[RESULT] 
{\sl \label{ncdq2} The NC $e^+p$ cross section  
${\rm d}\sigma_{NC}/{\rm d}Q^2$ for $y<0.9$ after 
correction ($k_{\rm cor}$) according to the  
Standard Model expectation for 
the kinematic cut $E_e^{\prime}>6$~GeV 
for $Q^2<890$~GeV$^2$. The 
statistical $(\delta_{stat})$, 
uncorrelated systematic $(\delta_{unc})$, 
correlated systematic $(\delta_{cor})$, 
and total $(\delta_{tot})$ errors are provided. 
In addition the correlated systematic  
error contributions from a 
positive variation of one  
standard deviation of the 
electron energy error ($\delta_{cor}^{E^+}$), of 
the polar electron angle error 
($\delta_{cor}^{\theta^+}$), of the hadronic 
energy error ($\delta_{cor}^{h^+}$), of the error 
due to noise subtraction ($\delta_{cor}^{N^+}$), and 
of the error due to background subtraction 
($\delta_{cor}^{B^+}$) are given. 
The normalisation uncertainty of 1.5\% is 
not included in the errors.} 
\end{table} 


==> add.tex <==
The measured value is scaled to the full kinematic region by applying
a simple scale factor determined from the QCD fit. No additional
uncertainty due to the scale factor is considered, and the
experimental value obtained is
$\int_0^1 {\rm d}x \,\, F_3^{\gamma Z} = 1.69 \pm 0.12 ({\rm stat})
\pm 0.10 ({\rm syst})$ 


==> combination_tables/p_1_xF3.tex <==
$ 60.00$ &$  0.001 $ &$ -0.013 $ &$ 0.011 $ &$ 0.025 $ &$ 0.017 $ &$0.032$  \\
$ 90.00$ &$  0.001 $ &$ -0.014 $ &$ 0.009 $ &$ 0.023 $ &$ 0.016 $ &$0.030$  \\
$ 100.00$ &$  0.001 $ &$ -0.047 $ &$ 0.024 $ &$ 0.056 $ &$ 0.020 $ &$0.065$  \\
$ 100.00$ &$  0.002 $ &$ -0.088 $ &$ 0.030 $ &$ 0.052 $ &$ 0.020 $ &$0.063$  \\
$ 120.00$ &$  0.002 $ &$  0.006 $ &$ 0.010 $ &$ 0.020 $ &$ 0.015 $ &$0.027$  \\
$ 120.00$ &$  0.002 $ &$ -0.013 $ &$ 0.008 $ &$ 0.012 $ &$ 0.016 $ &$0.022$  \\
$ 120.00$ &$  0.003 $ &$ -0.017 $ &$ 0.017 $ &$ 0.021 $ &$ 0.024 $ &$0.035$  \\
$ 150.00$ &$  0.002 $ &$ -0.025 $ &$ 0.011 $ &$ 0.020 $ &$ 0.014 $ &$0.027$  \\
$ 150.00$ &$  0.003 $ &$ -0.017 $ &$ 0.008 $ &$ 0.013 $ &$ 0.019 $ &$0.025$  \\
$ 150.00$ &$  0.005 $ &$  0.014 $ &$ 0.014 $ &$ 0.024 $ &$ 0.027 $ &$0.039$  \\
$ 150.00$ &$  0.008 $ &$ -0.029 $ &$ 0.028 $ &$ 0.054 $ &$ 0.040 $ &$0.073$  \\
$ 150.00$ &$  0.013 $ &$  0.031 $ &$ 0.061 $ &$ 0.135 $ &$ 0.060 $ &$0.159$  \\
$ 200.00$ &$  0.003 $ &$ -0.023 $ &$ 0.012 $ &$ 0.019 $ &$ 0.013 $ &$0.026$  \\
$ 200.00$ &$  0.003 $ &$ -0.006 $ &$ 0.012 $ &$ 0.010 $ &$ 0.014 $ &$0.021$  \\
$ 200.00$ &$  0.005 $ &$ -0.007 $ &$ 0.011 $ &$ 0.015 $ &$ 0.020 $ &$0.028$  \\
$ 200.00$ &$  0.008 $ &$ -0.005 $ &$ 0.016 $ &$ 0.029 $ &$ 0.029 $ &$0.044$  \\
$ 200.00$ &$  0.013 $ &$ -0.032 $ &$ 0.027 $ &$ 0.027 $ &$ 0.041 $ &$0.056$  \\
$ 200.00$ &$  0.020 $ &$ -0.039 $ &$ 0.040 $ &$ 0.048 $ &$ 0.057 $ &$0.084$  \\
$ 200.00$ &$  0.032 $ &$ -0.107 $ &$ 0.063 $ &$ 0.085 $ &$ 0.078 $ &$0.131$  \\
$ 200.00$ &$  0.050 $ &$  0.060 $ &$ 0.101 $ &$ 0.152 $ &$ 0.110 $ &$0.213$  \\
$ 200.00$ &$  0.080 $ &$  0.078 $ &$ 0.148 $ &$ 0.239 $ &$ 0.148 $ &$0.317$  \\
$ 200.00$ &$  0.130 $ &$ -0.042 $ &$ 0.239 $ &$ 0.358 $ &$ 0.206 $ &$0.477$  \\
$ 200.00$ &$  0.180 $ &$ -0.379 $ &$ 0.413 $ &$ 0.597 $ &$ 0.241 $ &$0.765$  \\
$ 250.00$ &$  0.003 $ &$ -0.015 $ &$ 0.014 $ &$ 0.019 $ &$ 0.013 $ &$0.027$  \\
$ 250.00$ &$  0.005 $ &$ -0.011 $ &$ 0.011 $ &$ 0.011 $ &$ 0.016 $ &$0.022$  \\
$ 250.00$ &$  0.008 $ &$ -0.001 $ &$ 0.015 $ &$ 0.018 $ &$ 0.023 $ &$0.033$  \\
$ 250.00$ &$  0.013 $ &$ -0.006 $ &$ 0.023 $ &$ 0.031 $ &$ 0.033 $ &$0.051$  \\
$ 250.00$ &$  0.020 $ &$ -0.053 $ &$ 0.031 $ &$ 0.044 $ &$ 0.045 $ &$0.070$  \\
$ 250.00$ &$  0.032 $ &$ -0.003 $ &$ 0.046 $ &$ 0.061 $ &$ 0.062 $ &$0.098$  \\
$ 250.00$ &$  0.050 $ &$ -0.138 $ &$ 0.069 $ &$ 0.084 $ &$ 0.084 $ &$0.137$  \\
$ 250.00$ &$  0.080 $ &$ -0.154 $ &$ 0.099 $ &$ 0.103 $ &$ 0.116 $ &$0.184$  \\
$ 250.00$ &$  0.130 $ &$ -0.003 $ &$ 0.145 $ &$ 0.228 $ &$ 0.158 $ &$0.313$  \\
$ 250.00$ &$  0.180 $ &$  0.304 $ &$ 0.257 $ &$ 0.451 $ &$ 0.188 $ &$0.552$  \\
$ 300.00$ &$  0.004 $ &$ -0.009 $ &$ 0.015 $ &$ 0.018 $ &$ 0.012 $ &$0.026$  \\
$ 300.00$ &$  0.005 $ &$  0.001 $ &$ 0.015 $ &$ 0.010 $ &$ 0.014 $ &$0.023$  \\
$ 300.00$ &$  0.008 $ &$  0.004 $ &$ 0.015 $ &$ 0.013 $ &$ 0.019 $ &$0.028$  \\
$ 300.00$ &$  0.013 $ &$  0.010 $ &$ 0.020 $ &$ 0.023 $ &$ 0.027 $ &$0.041$  \\
$ 300.00$ &$  0.020 $ &$ -0.040 $ &$ 0.031 $ &$ 0.031 $ &$ 0.038 $ &$0.058$  \\
$ 300.00$ &$  0.032 $ &$ -0.017 $ &$ 0.044 $ &$ 0.048 $ &$ 0.052 $ &$0.083$  \\
$ 300.00$ &$  0.050 $ &$  0.025 $ &$ 0.063 $ &$ 0.074 $ &$ 0.069 $ &$0.120$  \\
$ 300.00$ &$  0.080 $ &$ -0.276 $ &$ 0.093 $ &$ 0.108 $ &$ 0.097 $ &$0.172$  \\
$ 300.00$ &$  0.130 $ &$ -0.190 $ &$ 0.130 $ &$ 0.205 $ &$ 0.133 $ &$0.277$  \\
$ 300.00$ &$  0.180 $ &$ -0.394 $ &$ 0.225 $ &$ 0.406 $ &$ 0.160 $ &$0.491$  \\
$ 300.00$ &$  0.400 $ &$ -0.193 $ &$ 0.280 $ &$ 0.481 $ &$ 0.188 $ &$0.587$  \\
$ 400.00$ &$  0.005 $ &$ -0.022 $ &$ 0.015 $ &$ 0.018 $ &$ 0.011 $ &$0.026$  \\
$ 400.00$ &$  0.008 $ &$  0.023 $ &$ 0.014 $ &$ 0.011 $ &$ 0.015 $ &$0.023$  \\
$ 400.00$ &$  0.013 $ &$ -0.004 $ &$ 0.018 $ &$ 0.016 $ &$ 0.021 $ &$0.032$  \\
$ 400.00$ &$  0.020 $ &$ -0.012 $ &$ 0.025 $ &$ 0.027 $ &$ 0.028 $ &$0.046$  \\
$ 400.00$ &$  0.032 $ &$ -0.004 $ &$ 0.037 $ &$ 0.030 $ &$ 0.039 $ &$0.061$  \\
$ 400.00$ &$  0.050 $ &$ -0.045 $ &$ 0.053 $ &$ 0.046 $ &$ 0.051 $ &$0.087$  \\
$ 400.00$ &$  0.080 $ &$ -0.161 $ &$ 0.079 $ &$ 0.060 $ &$ 0.072 $ &$0.122$  \\
$ 400.00$ &$  0.130 $ &$  0.081 $ &$ 0.109 $ &$ 0.123 $ &$ 0.099 $ &$0.192$  \\
$ 400.00$ &$  0.180 $ &$ -0.038 $ &$ 0.184 $ &$ 0.258 $ &$ 0.119 $ &$0.339$  \\
$ 400.00$ &$  0.250 $ &$ -0.180 $ &$ 0.362 $ &$ 0.740 $ &$ 0.156 $ &$0.838$  \\
$ 400.00$ &$  0.400 $ &$ -0.259 $ &$ 0.242 $ &$ 0.322 $ &$ 0.145 $ &$0.428$  \\
$ 500.00$ &$  0.007 $ &$ -0.001 $ &$ 0.015 $ &$ 0.016 $ &$ 0.010 $ &$0.024$  \\
$ 500.00$ &$  0.008 $ &$ -0.001 $ &$ 0.018 $ &$ 0.009 $ &$ 0.011 $ &$0.023$  \\
$ 500.00$ &$  0.013 $ &$  0.017 $ &$ 0.019 $ &$ 0.013 $ &$ 0.017 $ &$0.028$  \\
$ 500.00$ &$  0.020 $ &$ -0.030 $ &$ 0.024 $ &$ 0.020 $ &$ 0.023 $ &$0.038$  \\
$ 500.00$ &$  0.032 $ &$  0.007 $ &$ 0.035 $ &$ 0.026 $ &$ 0.032 $ &$0.054$  \\


==> combination_tables/p_2_xF3.tex <==
$ 500.00$ &$  0.050 $ &$  0.056 $ &$ 0.050 $ &$ 0.040 $ &$ 0.044 $ &$0.077$  \\
$ 500.00$ &$  0.080 $ &$ -0.130 $ &$ 0.073 $ &$ 0.051 $ &$ 0.058 $ &$0.107$  \\
$ 500.00$ &$  0.130 $ &$ -0.032 $ &$ 0.118 $ &$ 0.098 $ &$ 0.082 $ &$0.174$  \\
$ 500.00$ &$  0.180 $ &$  0.370 $ &$ 0.154 $ &$ 0.152 $ &$ 0.098 $ &$0.238$  \\
$ 500.00$ &$  0.250 $ &$  0.079 $ &$ 0.209 $ &$ 0.223 $ &$ 0.114 $ &$0.326$  \\
$ 650.00$ &$  0.009 $ &$ -0.007 $ &$ 0.016 $ &$ 0.016 $ &$ 0.010 $ &$0.025$  \\
$ 650.00$ &$  0.013 $ &$  0.033 $ &$ 0.016 $ &$ 0.010 $ &$ 0.013 $ &$0.022$  \\
$ 650.00$ &$  0.020 $ &$  0.033 $ &$ 0.022 $ &$ 0.015 $ &$ 0.017 $ &$0.032$  \\
$ 650.00$ &$  0.032 $ &$  0.022 $ &$ 0.032 $ &$ 0.026 $ &$ 0.025 $ &$0.048$  \\
$ 650.00$ &$  0.050 $ &$  0.063 $ &$ 0.044 $ &$ 0.030 $ &$ 0.033 $ &$0.063$  \\
$ 650.00$ &$  0.080 $ &$  0.019 $ &$ 0.065 $ &$ 0.041 $ &$ 0.043 $ &$0.089$  \\
$ 650.00$ &$  0.130 $ &$ -0.257 $ &$ 0.106 $ &$ 0.078 $ &$ 0.062 $ &$0.145$  \\
$ 650.00$ &$  0.180 $ &$ -0.042 $ &$ 0.136 $ &$ 0.116 $ &$ 0.076 $ &$0.194$  \\
$ 650.00$ &$  0.250 $ &$  0.126 $ &$ 0.181 $ &$ 0.173 $ &$ 0.082 $ &$0.264$  \\
$ 650.00$ &$  0.400 $ &$ -0.603 $ &$ 0.226 $ &$ 0.200 $ &$ 0.078 $ &$0.312$  \\
$ 800.00$ &$  0.010 $ &$  0.014 $ &$ 0.018 $ &$ 0.015 $ &$ 0.009 $ &$0.026$  \\
$ 800.00$ &$  0.013 $ &$  0.038 $ &$ 0.021 $ &$ 0.009 $ &$ 0.010 $ &$0.025$  \\
$ 800.00$ &$  0.020 $ &$  0.019 $ &$ 0.020 $ &$ 0.011 $ &$ 0.013 $ &$0.026$  \\
$ 800.00$ &$  0.032 $ &$  0.017 $ &$ 0.029 $ &$ 0.020 $ &$ 0.019 $ &$0.040$  \\
$ 800.00$ &$  0.050 $ &$  0.049 $ &$ 0.043 $ &$ 0.024 $ &$ 0.027 $ &$0.056$  \\
$ 800.00$ &$  0.080 $ &$ -0.141 $ &$ 0.062 $ &$ 0.036 $ &$ 0.036 $ &$0.081$  \\
$ 800.00$ &$  0.130 $ &$ -0.049 $ &$ 0.098 $ &$ 0.064 $ &$ 0.048 $ &$0.127$  \\
$ 800.00$ &$  0.180 $ &$ -0.111 $ &$ 0.131 $ &$ 0.096 $ &$ 0.061 $ &$0.173$  \\
$ 800.00$ &$  0.250 $ &$ -0.024 $ &$ 0.160 $ &$ 0.124 $ &$ 0.064 $ &$0.212$  \\
$ 800.00$ &$  0.400 $ &$  0.030 $ &$ 0.198 $ &$ 0.180 $ &$ 0.059 $ &$0.274$  \\
$ 800.00$ &$  0.650 $ &$ -0.183 $ &$ 0.163 $ &$ 0.110 $ &$ 0.035 $ &$0.200$  \\
$ 1000.00$ &$  0.013 $ &$  0.015 $ &$ 0.017 $ &$ 0.011 $ &$ 0.008 $ &$0.022$  \\
$ 1000.00$ &$  0.020 $ &$  0.021 $ &$ 0.019 $ &$ 0.009 $ &$ 0.011 $ &$0.023$  \\
$ 1000.00$ &$  0.032 $ &$  0.036 $ &$ 0.026 $ &$ 0.014 $ &$ 0.015 $ &$0.033$  \\
$ 1000.00$ &$  0.050 $ &$ -0.047 $ &$ 0.036 $ &$ 0.024 $ &$ 0.021 $ &$0.048$  \\
$ 1000.00$ &$  0.080 $ &$ -0.038 $ &$ 0.055 $ &$ 0.027 $ &$ 0.029 $ &$0.068$  \\
$ 1000.00$ &$  0.130 $ &$  0.009 $ &$ 0.092 $ &$ 0.049 $ &$ 0.040 $ &$0.111$  \\
$ 1000.00$ &$  0.180 $ &$  0.219 $ &$ 0.117 $ &$ 0.071 $ &$ 0.048 $ &$0.145$  \\
$ 1000.00$ &$  0.250 $ &$  0.266 $ &$ 0.146 $ &$ 0.099 $ &$ 0.055 $ &$0.185$  \\
$ 1000.00$ &$  0.400 $ &$  0.007 $ &$ 0.179 $ &$ 0.139 $ &$ 0.048 $ &$0.232$  \\
$ 1200.00$ &$  0.013 $ &$  0.023 $ &$ 0.027 $ &$ 0.014 $ &$ 0.008 $ &$0.032$  \\
$ 1200.00$ &$  0.020 $ &$  0.037 $ &$ 0.019 $ &$ 0.009 $ &$ 0.009 $ &$0.023$  \\
$ 1200.00$ &$  0.032 $ &$  0.066 $ &$ 0.025 $ &$ 0.010 $ &$ 0.013 $ &$0.030$  \\
$ 1200.00$ &$  0.050 $ &$  0.061 $ &$ 0.034 $ &$ 0.017 $ &$ 0.017 $ &$0.042$  \\
$ 1200.00$ &$  0.080 $ &$  0.031 $ &$ 0.051 $ &$ 0.025 $ &$ 0.024 $ &$0.062$  \\
$ 1200.00$ &$  0.130 $ &$ -0.068 $ &$ 0.088 $ &$ 0.046 $ &$ 0.032 $ &$0.104$  \\
$ 1200.00$ &$  0.180 $ &$ -0.095 $ &$ 0.111 $ &$ 0.056 $ &$ 0.040 $ &$0.131$  \\
$ 1200.00$ &$  0.250 $ &$ -0.353 $ &$ 0.130 $ &$ 0.074 $ &$ 0.042 $ &$0.156$  \\
$ 1200.00$ &$  0.400 $ &$  0.194 $ &$ 0.144 $ &$ 0.115 $ &$ 0.036 $ &$0.188$  \\
$ 1500.00$ &$  0.020 $ &$  0.057 $ &$ 0.019 $ &$ 0.011 $ &$ 0.007 $ &$0.023$  \\
$ 1500.00$ &$  0.032 $ &$  0.066 $ &$ 0.025 $ &$ 0.009 $ &$ 0.010 $ &$0.028$  \\
$ 1500.00$ &$  0.050 $ &$  0.020 $ &$ 0.032 $ &$ 0.013 $ &$ 0.014 $ &$0.037$  \\
$ 1500.00$ &$  0.080 $ &$  0.114 $ &$ 0.047 $ &$ 0.021 $ &$ 0.020 $ &$0.055$  \\
$ 1500.00$ &$  0.130 $ &$  0.038 $ &$ 0.077 $ &$ 0.036 $ &$ 0.024 $ &$0.088$  \\
$ 1500.00$ &$  0.180 $ &$ -0.111 $ &$ 0.096 $ &$ 0.046 $ &$ 0.030 $ &$0.110$  \\
$ 1500.00$ &$  0.250 $ &$  0.006 $ &$ 0.112 $ &$ 0.064 $ &$ 0.033 $ &$0.133$  \\
$ 1500.00$ &$  0.400 $ &$  0.083 $ &$ 0.132 $ &$ 0.091 $ &$ 0.029 $ &$0.163$  \\
$ 1500.00$ &$  0.650 $ &$ -0.011 $ &$ 0.048 $ &$ 0.029 $ &$ 0.006 $ &$0.056$  \\
$ 2000.00$ &$  0.022 $ &$  0.081 $ &$ 0.031 $ &$ 0.014 $ &$ 0.007 $ &$0.035$  \\
$ 2000.00$ &$  0.032 $ &$  0.057 $ &$ 0.021 $ &$ 0.009 $ &$ 0.007 $ &$0.023$  \\
$ 2000.00$ &$  0.050 $ &$  0.024 $ &$ 0.029 $ &$ 0.010 $ &$ 0.010 $ &$0.032$  \\
$ 2000.00$ &$  0.080 $ &$  0.058 $ &$ 0.038 $ &$ 0.016 $ &$ 0.013 $ &$0.044$  \\
$ 2000.00$ &$  0.130 $ &$ -0.031 $ &$ 0.064 $ &$ 0.026 $ &$ 0.018 $ &$0.071$  \\
$ 2000.00$ &$  0.180 $ &$ -0.090 $ &$ 0.083 $ &$ 0.036 $ &$ 0.023 $ &$0.094$  \\
$ 2000.00$ &$  0.250 $ &$  0.016 $ &$ 0.095 $ &$ 0.049 $ &$ 0.025 $ &$0.110$  \\
$ 2000.00$ &$  0.400 $ &$  0.018 $ &$ 0.102 $ &$ 0.065 $ &$ 0.021 $ &$0.123$  \\


==> combination_tables/p_3_xF3.tex <==
$ 2000.00$ &$  0.650 $ &$ -0.093 $ &$ 0.039 $ &$ 0.022 $ &$ 0.004 $ &$0.045$  \\
$ 3000.00$ &$  0.032 $ &$  0.061 $ &$ 0.017 $ &$ 0.009 $ &$ 0.006 $ &$0.021$  \\
$ 3000.00$ &$  0.050 $ &$  0.053 $ &$ 0.016 $ &$ 0.008 $ &$ 0.007 $ &$0.019$  \\
$ 3000.00$ &$  0.080 $ &$  0.067 $ &$ 0.024 $ &$ 0.010 $ &$ 0.009 $ &$0.028$  \\
$ 3000.00$ &$  0.130 $ &$  0.122 $ &$ 0.038 $ &$ 0.018 $ &$ 0.013 $ &$0.044$  \\
$ 3000.00$ &$  0.180 $ &$ -0.022 $ &$ 0.052 $ &$ 0.024 $ &$ 0.015 $ &$0.059$  \\
$ 3000.00$ &$  0.250 $ &$  0.062 $ &$ 0.057 $ &$ 0.028 $ &$ 0.016 $ &$0.065$  \\
$ 3000.00$ &$  0.400 $ &$ -0.022 $ &$ 0.058 $ &$ 0.040 $ &$ 0.013 $ &$0.072$  \\
$ 3000.00$ &$  0.650 $ &$ -0.020 $ &$ 0.021 $ &$ 0.013 $ &$ 0.003 $ &$0.024$  \\
$ 5000.00$ &$  0.055 $ &$  0.081 $ &$ 0.020 $ &$ 0.009 $ &$ 0.005 $ &$0.022$  \\
$ 5000.00$ &$  0.080 $ &$  0.084 $ &$ 0.016 $ &$ 0.007 $ &$ 0.005 $ &$0.018$  \\
$ 5000.00$ &$  0.130 $ &$  0.140 $ &$ 0.026 $ &$ 0.012 $ &$ 0.008 $ &$0.030$  \\
$ 5000.00$ &$  0.180 $ &$  0.157 $ &$ 0.034 $ &$ 0.015 $ &$ 0.009 $ &$0.038$  \\
$ 5000.00$ &$  0.250 $ &$  0.036 $ &$ 0.045 $ &$ 0.022 $ &$ 0.009 $ &$0.051$  \\
$ 5000.00$ &$  0.400 $ &$  0.006 $ &$ 0.041 $ &$ 0.021 $ &$ 0.007 $ &$0.047$  \\
$ 5000.00$ &$  0.650 $ &$  0.023 $ &$ 0.014 $ &$ 0.007 $ &$ 0.001 $ &$0.016$  \\
$ 8000.00$ &$  0.088 $ &$  0.141 $ &$ 0.028 $ &$ 0.010 $ &$ 0.005 $ &$0.030$  \\
$ 8000.00$ &$  0.130 $ &$  0.155 $ &$ 0.022 $ &$ 0.010 $ &$ 0.005 $ &$0.025$  \\
$ 8000.00$ &$  0.180 $ &$  0.090 $ &$ 0.027 $ &$ 0.011 $ &$ 0.005 $ &$0.030$  \\
$ 8000.00$ &$  0.250 $ &$  0.058 $ &$ 0.034 $ &$ 0.012 $ &$ 0.006 $ &$0.036$  \\
$ 8000.00$ &$  0.400 $ &$  0.055 $ &$ 0.032 $ &$ 0.017 $ &$ 0.004 $ &$0.036$  \\
$ 8000.00$ &$  0.650 $ &$ -0.009 $ &$ 0.011 $ &$ 0.005 $ &$ 0.001 $ &$0.012$  \\
$ 12000.00$ &$  0.130 $ &$  0.255 $ &$ 0.048 $ &$ 0.016 $ &$ 0.004 $ &$0.051$  \\
$ 12000.00$ &$  0.180 $ &$  0.169 $ &$ 0.027 $ &$ 0.008 $ &$ 0.004 $ &$0.028$  \\
$ 12000.00$ &$  0.250 $ &$  0.141 $ &$ 0.026 $ &$ 0.008 $ &$ 0.003 $ &$0.028$  \\
$ 12000.00$ &$  0.400 $ &$  0.142 $ &$ 0.030 $ &$ 0.014 $ &$ 0.003 $ &$0.033$  \\
$ 12000.00$ &$  0.650 $ &$ -0.005 $ &$ 0.011 $ &$ 0.004 $ &$ 0.001 $ &$0.012$  \\
$ 20000.00$ &$  0.250 $ &$  0.184 $ &$ 0.030 $ &$ 0.007 $ &$ 0.003 $ &$0.031$  \\
$ 20000.00$ &$  0.400 $ &$  0.112 $ &$ 0.025 $ &$ 0.008 $ &$ 0.002 $ &$0.026$  \\
$ 20000.00$ &$  0.650 $ &$  0.007 $ &$ 0.009 $ &$ 0.004 $ &$ 0.000 $ &$0.010$  \\
$ 30000.00$ &$  0.400 $ &$  0.069 $ &$ 0.032 $ &$ 0.007 $ &$ 0.002 $ &$0.032$  \\
$ 30000.00$ &$  0.650 $ &$  0.031 $ &$ 0.013 $ &$ 0.004 $ &$ 0.000 $ &$0.013$  \\

